The Free Transformer

We propose an extension of the decoder Transformer that conditions its generative process on random latent variables which are learned without supervision thanks to a variational procedure. Experimental evaluations show that allowing such a conditioning translates into substantial improvements on downstream tasks.

==> 8B_1T_tasks_perfs.tex <==
\hline
\multicolumn{4}{c}{Generative code/math}\\
\hline
human\_eval\_plu (pass@1) & 0.268 & 0.299 & \colorbox{green}{+11.36\%}\\
mbpp (pass@1) & 0.428 & 0.440 & \colorbox{green!25}{+2.80\%}\\
gsm8k (em) & 0.321 & 0.331 & \colorbox{green!25}{+2.83\%}\\
\hline
\multicolumn{4}{c}{Multi-choice general knowledge / common sense}\\
\hline
mmlu (macro\_avg/acc\_char) & 0.592 & 0.623 & \colorbox{green!25}{+5.20\%}\\
csqa (acc\_char) & 0.707 & 0.748 & \colorbox{green!25}{+5.79\%}\\
hellaswag (acc\_char) & 0.799 & 0.799 & \colorbox{white}{-0.01\%}\\
winogrande (acc\_char) & 0.739 & 0.735 & \colorbox{white}{-0.53\%}\\
obqa (acc\_completion) & 0.564 & 0.562 & \colorbox{white}{-0.35\%}\\
arc\_challenge (acc\_completion) & 0.542 & 0.535 & \colorbox{red!10}{-1.42\%}\\
arc\_easy (acc\_completion) & 0.721 & 0.711 & \colorbox{red!10}{-1.41\%}\\
piqa (acc\_char) & 0.805 & 0.812 & \colorbox{white}{+0.88\%}\\
\hline
\multicolumn{4}{c}{Multi-choice text understanding}\\
\hline
race.high (acc\_char) & 0.473 & 0.463 & \colorbox{red!10}{-2.06\%}\\
race.middle (acc\_char) & 0.632 & 0.634 & \colorbox{white}{+0.33\%}\\
boolq (acc\_completion) & 0.713 & 0.725 & \colorbox{green!25}{+1.63\%}\\
\hline
\multicolumn{4}{c}{Culture}\\
\hline
nq (em) & 0.248 & 0.247 & \colorbox{white}{-0.22\%}\\
tqa (em) & 0.583 & 0.577 & \colorbox{red!10}{-1.00\%}


==> 8B_1T_tasks_perfs_ave_20.tex <==
\hline
\multicolumn{4}{c}{Generative code/math}\\
\hline
human\_eval\_plu (pass@1) & 0.245 & 0.256 & \colorbox{green!25}{+4.22\%}\\
mbpp (pass@1) & 0.396 & 0.421 & \colorbox{green!25}{+6.08\%}\\
gsm8k (em) & 0.280 & 0.296 & \colorbox{green!25}{+5.84\%}\\
\hline
\multicolumn{4}{c}{Multi-choice general knowledge / common sense}\\
\hline
mmlu (macro\_avg/acc\_char) & 0.567 & 0.596 & \colorbox{green!25}{+5.16\%}\\
csqa (acc\_char) & 0.689 & 0.733 & \colorbox{green!25}{+6.28\%}\\
hellaswag (acc\_char) & 0.787 & 0.788 & \colorbox{white}{+0.18\%}\\
winogrande (acc\_char) & 0.725 & 0.727 & \colorbox{white}{+0.27\%}\\
obqa (acc\_completion) & 0.556 & 0.551 & \colorbox{white}{-0.86\%}\\
arc\_challenge (acc\_completion) & 0.524 & 0.522 & \colorbox{white}{-0.40\%}\\
arc\_easy (acc\_completion) & 0.706 & 0.711 & \colorbox{white}{+0.68\%}\\
piqa (acc\_char) & 0.802 & 0.807 & \colorbox{white}{+0.61\%}\\
\hline
\multicolumn{4}{c}{Multi-choice text understanding}\\
\hline
race.high (acc\_char) & 0.467 & 0.460 & \colorbox{red!10}{-1.55\%}\\
race.middle (acc\_char) & 0.623 & 0.624 & \colorbox{white}{+0.16\%}\\
boolq (acc\_completion) & 0.755 & 0.754 & \colorbox{white}{-0.10\%}\\
\hline
\multicolumn{4}{c}{Culture}\\
\hline
nq (em) & 0.229 & 0.227 & \colorbox{white}{-0.76\%}\\
tqa (em) & 0.549 & 0.544 & \colorbox{white}{-0.90\%}

